A well-quasi-order for continuous functions

We prove that continuous reducibility is a well-quasi-order on the class of continuous functions between separable metrizable spaces with analytic zero-dimensional domain. To achieve this, we define scattered functions, which generalize scattered spaces, and describe exhaustively scattered functions between zero-dimensional separable metrizable spaces up to continuous equivalence.

==> 01_acknowledgments.tex <==
% !TEX root = _main_memo.tex



==> macros-rep.tex <==
% !TEX encoding = UTF-8 Unicode

\newcommand{\trel}{\rightrightarrows}


\newcommand{\bsc}[1]{\mathbf{\Sigma}^{0}_{#1}} %Boldface(borel) borel sigma class
\newcommand{\bpc}[1]{%Boldface borel pi class
\mathbf{\Pi}^{0}_{#1}} 
\newcommand{\bdc}[1]{%Boldface borel delta class
\mathbf{\Delta}^{0}_{#1}} 

%\DeclareMathOperator{\wbdc}{\twoheaddownarrow}
%\DeclareMathOperator{\wbuc}{\twoheaduparrow}

\newcommand{\ISeq}[1][\finSub]{I^{<\omega}(#1)}

\newcommand{\Power}{\mathcal{P}\omega}
\newcommand{\PowerFin}{\mathcal{P}_{<\infty}(\omega)}
\newcommand{\PowerInf}{\mathcal{P}_{\infty}\omega}


\newcommand{\rbij}[1]{\left\langle #1 \right\rangle}%recursive bijection from some \omega^{k} to \omega

\newcommand{\I}{\mathrm{I}}
\newcommand{\II}{\mathrm{II}}


\newcommand{\squb} {\sqsubseteq}

%\newcommand{\Conc}{\omega^{\leq\omega}}
\newcommand{\lW}{\leqslant_{\textrm{W}}}
\newcommand{\notlW}{\nleqslant_{\textrm{W}}}
\newcommand{\We}{\equiv_{\textrm{W}}}
\newcommand{\lC}{\leq_C}


\newcommand{\WrF}{\leq^{\textrm{rep}}}
\newcommand{\Mr}{\preccurlyeq_{\textrm{W}}}
\newcommand{\nMr}{\not\preccurlyeq_{\textrm{W}}}

\newcommand{\vEMSB}{\mathfrak{L}^{B}}
\newcommand{\GL}{G}
\newcommand{\leqvEMSB}{\leq_{\mathfrak{L}}}
\newcommand{\nleqvEMSB}{\nleq_{\mathfrak{L}}}

\newcommand{\vEMSLip}{B_\textrm{Lip}}
\newcommand{\leqvEMSLip}{\leq_{\textrm{Lip}}}
\newcommand{\nleqvEMSLip}{\nleq_{\textrm{Lip}}}
\newcommand{\GLip}{G_{\text{Lip}}}


\newcommand{\vEMS}{B}
\newcommand{\leqvEMS}{\leq_{\text{c}}}
\newcommand{\nleqvEMS}{\nleq_{\text{c}}}

\newcommand{\vEMSg}{B^{\text{gen}}}
\newcommand{\leqvEMSg}{\preccurlyeq_{\text{c}}}
\newcommand{\nleqvEMSg}{\not\preccurlyeq_{\text{c}}}


\newcommand{\NowAsc}{L^{\text{na}}}

\newcommand{\body}[1]{\left[#1\right]}
 




\newcommand{\symd}{\mathbin{\triangle}}

\newcommand{\onto}{\twoheadrightarrow}

 
 \newcommand{\qqand}{\qquad\mbox{ and }\qquad}
 
 
 %%%%%
 
 \DeclareMathOperator{\Pt}{Pt}
\DeclareMathOperator{\Open}{\Omega}
\newcommand{\Frm}{\textbf{Frm}}
\newcommand{\Top}{\textbf{Top}}
\newcommand{\Sob}{\textbf{Sob}}
\newcommand{\sFrm}{\textbf{sFrm}}


==> macros.tex <==










%%%%%%%

%\theoremstyle{plain} 
%\newtheorem{theorem}{Theorem}[chapter] 
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{ppt}[theorem]{Properties}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{conjecture} {Conjecture}
%\newtheorem{fact}[theorem]{Fact}
%\newtheorem{facts}[theorem]{Facts}
%
%
%\newtheorem*{claim*}{Claim}
%\newtheorem{thm}[theorem]{Theorem}
%\newtheorem{prop}[theorem]{Proposition}
%\newtheorem{cor}[theorem]{Corollary}
%\newtheorem{pp}[theorem]{Properties}
%\newtheorem{lem}[theorem]{Lemma}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{scholium}[theorem]{Scholium}
%\newtheorem{maintheorem}{Main Theorem}
%\newtheorem{question} {Question}
%
%\crefname{maintheorem}{Main Theorem}{Main Theorems}
%\crefname{fact}{Fact}{Facts}
%
%
%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}	
%\newtheorem{defns}[theorem]{Definitions}	
%\newtheorem{defn}[theorem]{Definition}	
%
%\theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem*{remark*}{Remark}
%\newtheorem{rem}[theorem]{Remark}
%\newtheorem{rems}[theorem]{Remarks}
%\newtheorem{remarks}[theorem]{Remarks}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{ex}[theorem]{Example}
%\newtheorem*{conv} {Convention} 
%\newtheorem*{nota} {Notation} % * signifie que ces paragraphes ne seront pas numérotés
%\newtheorem*{notas} {Notations}
%
%
%
%
%%\newtheorem*{conv} {Convention} 
%%\newtheorem*{nota} {Notation} 
%%\newtheorem*{notas} {Notations} 
%\newtheorem*{note}{Note}
%%\newtheorem*{expl} {Explication}
%%\newtheorem*{quest} {Question}
%
%%Create Uppercase aliases when we need to avoid page break after theorem title, for example for theorems with lists
%%it requires needspace package
%
%\newenvironment{Theorem}{%
%    \Needspace*{3\baselineskip}%     \Needspace*{3\baselineskip}%
%    \theorem
%}{\endtheorem}
%
%\newenvironment{Proposition}{%
%    \Needspace*{2\baselineskip}%
%    \proposition
%}{\endproposition}
%
%\newenvironment{Fact}{%
%    \Needspace*{5\baselineskip}%
%    \fact
%}{\endfact}
%
%\newenvironment{Corollary}{%
%    \Needspace*{2\baselineskip}%
%    \corollary
%}{\endcorollary}

%%%% Proof environnement
%% When trouble with the qed symbol one solution is to put
%% \belowdisplayskip=-12pt  the last align or split environnement.

\newcommand{\smileyqed}{\tikz[baseline=-0.75ex,black]{
\draw[xshift=-1.35mm, yshift=-1.35mm] rectangle (2.7mm,2.7mm); %\draw (-1,-1) -- (-1,1) -- (1,1) -- (1,-1) -- (-1,-1);
\node[fill,circle,inner sep=0.5pt] (left eye) at (135:0.8mm) {};
\node[fill,circle,inner sep=0.5pt] (right eye) at (45:0.8mm) {};
\draw (-145:0.9mm) arc (-120:-60:1.5mm);
    }
}

% \renewcommand{\qedsymbol}{$\smileyqed$}

%\newlist{enumThm}{enumerate}{2}% enumerate in Definitions
%\setlist[enumThm,1]{label=\upshape(\roman*)}%beginpenalty=4,
%\setlist[enumThm,2]{label=\upshape(\alph*)}




\newlist{enumDefn}{enumerate}{2}% enumerate in Definitions
\setlist[enumDefn,1]{label=(\arabic*)}
\setlist[enumDefn,2]{label=(\arabic{enumDefni}\alph*),leftmargin=3em}

\newlist{enumRems}{enumerate}{1}% enumerate in Definitions
\setlist[enumRems,1]{label=\upshape(\arabic*)}

\newlist{itemProof}{itemize}{1}% itemize in Proofs
\setlist[itemProof]{label=--}

\newlist{enumProof}{enumerate}{1}% itemize in Proofs
\setlist[enumProof,1]{label=\upshape(\alph*)}

\newlist{enumProofParameter}{enumerate}{1}% itemize in Proofs
\setlist[enumProofParameter,1]{label=\upshape(\alph*)$_{\xi}$}

\newcommand*{\addsemicolon}[1]{#1:}
\newlist{descThm}{description}{1}% Desc in Thm statement
\setlist[descThm]{font=\normalfont}



\newlist{descProof}{description}{1}% Desc in proof statement
\setlist[descProof]{font={\normalfont\itshape}}


%%%%Pour résoudre le problème des thms commencant par une liste, pour que le premier item ne soit pas sur la même ligne que l'entête du thm
%
\makeatletter
\def\enumfix{%
\if@inlabel
 \noindent\par\nobreak\vskip-\parskip\vskip-\parskip\hrule\@height\z@
\fi}
%
%\let\oldenumThm\enumThm
%\def\enumThm{\enumfix\oldenumThm}
%
%\let\oldenumRems\enumRems
%\def\enumRems{\enumfix\oldenumRems}
%
%\let\oldenumDefn\enumDefn
%\def\enumDefn{\enumfix\oldenumDefn}
%
%\let\olditemize\itemize
%\def\itemize{\enumfix\olditemize}
%
%\makeatother
%%%%%%%%%


%\if@cref@capitalise
%\crefname{prop}{Proposition}{Propositions}
%\else
%\crefname{prop}{proposition}{propositions}
%\fi
%
%\Crefname{prop}{Proposition}{Propositions}

%\crefmultiformat{prop}{propositions~#2#1#3} { and~#2#1#3}{, #2#1#3}{ and~#2#1#3}
%\Crefmultiformat{prop}{Propositions~#2#1#3} { and~#2#1#3}{, #2#1#3}{ and~#2#1#3}
 \makeatletter
\if@cref@capitalise

\crefname{section}{Section}{Sections}
\crefname{subsection}{Subsection}{Subsections}
\crefname{equation}{}{}

\else

\crefname{section}{section}{sections}
\crefname{subsection}{subsection}{subsections}
\crefname{equation}{}{}

\fi


%\let\orgdescriptionlabel\descriptionlabel
%\renewcommand*{\descriptionlabel}[1]{%
%  \let\orglabel\label
%  \let\label\@gobble
%  \phantomsection
%  \edef\@currentlabel{#1}%
%  %\edef\@currentlabelname{#1}%
%  \let\label\orglabel
%  \orgdescriptionlabel{#1}%
%}

\makeatother

\Crefname{section}{Section}{Sections}
\Crefname{subsection}{Subsection}{Subsections}
\Crefname{equation}{}{}

\crefformat{enumDefni}{#2#1#3}
 \Crefformat{enumDefni}{#2#1#3}
\crefname{enumDefni}{}{}
\crefrangeformat{enumDefni}{#3#1#4--#5#2#6}

\crefformat{enumDefnii}{#2#1#3}
 \Crefformat{enumDefnii}{#2#1#3}
\crefname{enumDefnii}{}{}
 
 \crefformat{enumThmi}{#2#1#3}
 \Crefformat{enumThmi}{#2#1#3}
\crefname{enumThmi}{}{}

 \crefformat{enumThmii}{#2#1#3}
 \Crefformat{enumThmii}{#2#1#3}
\crefname{enumThmii}{}{}

 \crefformat{enumProofi}{#2#1#3}
 \Crefformat{enumProofi}{#2#1#3}
\crefname{enumThmi}{}{}
 
%\newenvironment{enumThm}{% enumerate in all AMS Thm env, prop, lem, thm...
%\begin{enumerate}[\upshape (i)]}
%{%
%\end{enumerate}
%}



==> macros_lms.tex <==










%%%%%%%

%\theoremstyle{plain} 
\newtheorem{theorem}{Theorem}[section] 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{ppt}[theorem]{Properties}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture} {Conjecture}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{facts}[theorem]{Facts}


%\newtheorem*{claim*}{Claim}
\newtheorem{thm}[theorem]{Theorem}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{pp}[theorem]{Properties}
\newtheorem{lem}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{scholium}[theorem]{Scholium}
\newtheorem{maintheorem}{Main Theorem}
\newtheorem{question} {Question}

\crefname{maintheorem}{Main Theorem}{Main Theorems}
\crefname{fact}{Fact}{Facts}


%\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}	
\newtheorem{defns}[theorem]{Definitions}	
\newtheorem{defn}[theorem]{Definition}	

%\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
%\newtheorem*{remark*}{Remark}
\newtheorem{rem}[theorem]{Remark}
\newtheorem{rems}[theorem]{Remarks}
\newtheorem{remarks}[theorem]{Remarks}
\newtheorem{example}[theorem]{Example}
\newtheorem{ex}[theorem]{Example}
%\newtheorem*{conv} {Convention} 
%\newtheorem*{nota} {Notation} % * signifie que ces paragraphes ne seront pas numérotés
%\newtheorem*{notas} {Notations}




%\newtheorem*{conv} {Convention} 
%\newtheorem*{nota} {Notation} 
%\newtheorem*{notas} {Notations} 
%\newtheorem*{note}{Note}
%\newtheorem*{expl} {Explication}
%\newtheorem*{quest} {Question}

%Create Uppercase aliases when we need to avoid page break after theorem title, for example for theorems with lists
%it requires needspace package

\newenvironment{Theorem}{%
    \Needspace*{2\baselineskip}%     \Needspace*{3\baselineskip}%
    \theorem
}{\endtheorem}

\newenvironment{Proposition}{%
    \Needspace*{2\baselineskip}%
    \proposition
}{\endproposition}

\newenvironment{Fact}{%
    \Needspace*{5\baselineskip}%
    \fact
}{\endfact}

\newenvironment{Corollary}{%
    \Needspace*{2\baselineskip}%
    \corollary
}{\endcorollary}

%%%% Proof environnement
%% When trouble with the qed symbol one solution is to put
%% \belowdisplayskip=-12pt  the last align or split environnement.

\newcommand{\smileyqed}{\tikz[baseline=-0.75ex,black]{
\draw[xshift=-1.35mm, yshift=-1.35mm] rectangle (2.7mm,2.7mm); %\draw (-1,-1) -- (-1,1) -- (1,1) -- (1,-1) -- (-1,-1);
\node[fill,circle,inner sep=0.5pt] (left eye) at (135:0.8mm) {};
\node[fill,circle,inner sep=0.5pt] (right eye) at (45:0.8mm) {};
\draw (-145:0.9mm) arc (-120:-60:1.5mm);
    }
}

%\renewcommand{\qedsymbol}{$\smileyqed$}

\newlist{enumThm}{enumerate}{2}% enumerate in Definitions
\setlist[enumThm,1]{label=\upshape(\roman*)}%beginpenalty=4,
\setlist[enumThm,2]{label=\upshape(\alph*)}




\newlist{enumDefn}{enumerate}{2}% enumerate in Definitions
\setlist[enumDefn,1]{label=(\arabic*)}
\setlist[enumDefn,2]{label=(\arabic{enumDefni}\alph*),leftmargin=3em}

\newlist{enumRems}{enumerate}{1}% enumerate in Definitions
\setlist[enumRems,1]{label=\upshape(\arabic*)}

\newlist{itemProof}{itemize}{1}% itemize in Proofs
\setlist[itemProof]{label=--}

\newlist{enumProof}{enumerate}{1}% itemize in Proofs
\setlist[enumProof,1]{label=\upshape(\alph*)}

\newlist{enumProofParameter}{enumerate}{1}% itemize in Proofs
\setlist[enumProofParameter,1]{label=\upshape(\alph*)$_{\xi}$}


\newlist{descThm}{description}{1}% Desc in Thm statement
\setlist[descThm]{font=\normalfont}

\newlist{descProof}{description}{1}% Desc in proof statement
\setlist[descProof]{font={\normalfont\itshape}}


%%%%Pour résoudre le problème des thms commencant par une liste, pour que le premier item ne soit pas sur la même ligne que l'entête du thm
%
\makeatletter
\def\enumfix{%
\if@inlabel
 \noindent\par\nobreak\vskip-\parskip\vskip-\parskip\hrule\@height\z@
\fi}
%
%\let\oldenumThm\enumThm
%\def\enumThm{\enumfix\oldenumThm}
%
%\let\oldenumRems\enumRems
%\def\enumRems{\enumfix\oldenumRems}
%
%\let\oldenumDefn\enumDefn
%\def\enumDefn{\enumfix\oldenumDefn}
%
%\let\olditemize\itemize
%\def\itemize{\enumfix\olditemize}
%
%\makeatother
%%%%%%%%%


%\if@cref@capitalise
%\crefname{prop}{Proposition}{Propositions}
%\else
%\crefname{prop}{proposition}{propositions}
%\fi
%
%\Crefname{prop}{Proposition}{Propositions}

%\crefmultiformat{prop}{propositions~#2#1#3} { and~#2#1#3}{, #2#1#3}{ and~#2#1#3}
%\Crefmultiformat{prop}{Propositions~#2#1#3} { and~#2#1#3}{, #2#1#3}{ and~#2#1#3}
\makeatletter
\if@cref@capitalise

\crefname{section}{Section}{Sections}
\crefname{subsection}{Subsection}{Subsections}
\crefname{equation}{}{}

\else

\crefname{section}{section}{sections}
\crefname{subsection}{subsection}{subsections}
\crefname{equation}{}{}

\fi


%\let\orgdescriptionlabel\descriptionlabel
%\renewcommand*{\descriptionlabel}[1]{%
%  \let\orglabel\label
%  \let\label\@gobble
%  \phantomsection
%  \edef\@currentlabel{#1}%
%  %\edef\@currentlabelname{#1}%
%  \let\label\orglabel
%  \orgdescriptionlabel{#1}%
%}

\makeatother

\Crefname{section}{Section}{Sections}
\Crefname{subsection}{Subsection}{Subsections}
\Crefname{equation}{}{}

\crefformat{enumDefni}{#2#1#3}
 \Crefformat{enumDefni}{#2#1#3}
\crefname{enumDefni}{}{}
\crefrangeformat{enumDefni}{#3#1#4--#5#2#6}

\crefformat{enumDefnii}{#2#1#3}
 \Crefformat{enumDefnii}{#2#1#3}
\crefname{enumDefnii}{}{}
 
 \crefformat{enumThmi}{#2#1#3}
 \Crefformat{enumThmi}{#2#1#3}
\crefname{enumThmi}{}{}

 \crefformat{enumThmii}{#2#1#3}
 \Crefformat{enumThmii}{#2#1#3}
\crefname{enumThmii}{}{}

 \crefformat{enumProofi}{#2#1#3}
 \Crefformat{enumProofi}{#2#1#3}
\crefname{enumThmi}{}{}
 
%\newenvironment{enumThm}{% enumerate in all AMS Thm env, prop, lem, thm...
%\begin{enumerate}[\upshape (i)]}
%{%
%\end{enumerate}
%}



==> macrosthmref_old.tex <==
% !TEX encoding = UTF-8 Unicode


%%%%%%%
\newtheorem{sharedtheoremcounter}{sharedtheoremcounter}[chapter] % dummy theorem type to act as shared counter
\NewDocumentCommand{\newzctheorem}{mO{#1}m}{
  \newtheorem{#1}[sharedtheoremcounter]{#3}
    \AddToHook{env/#1/begin}{%
      \zcsetup{countertype={sharedtheoremcounter=#2}}}
}



\theoremstyle{plain} 
\newzctheorem{maintheorem}{Main Theorem}
%}
%\zcsetup{countertype={theorem=theorem}}
\newzctheorem{theorem}[theorem]{Theorem}

%\AddToHook{env/proposition/begin}{%
\newzctheorem{proposition}[theorem]{Proposition}
%\AddToHook{env/corollary/begin}{%
\newzctheorem{corollary} [theorem]{Corollary}
%\newzctheorem{pp} {Properties}
%\AddToHook{env/lemma/begin}{%
\newzctheorem{lemma} [theorem]{Lemma}
\newzctheorem{conjecture} {Conjecture}
%\AddToHook{env/fact/begin}{%
\newtheorem{fact}[theorem]{Fact}
%\newzctheorem{facts}{Facts}
\newtheorem*{claim}{Claim}
%\newzctheorem*{xfact}{Fact}


\theoremstyle{definition}
%\AddToHook{env/definition/begin}{%
\newzctheorem{definition}[theorem]{Definition}	

\theoremstyle{remark}
%\AddToHook{env/remark/begin}{%
\newzctheorem{remark}[theorem]{Remark}
%\AddToHook{env/remarks/begin}{%
\newzctheorem{remarks}[theorem]{Remarks}
%\AddToHook{env/example/begin}{%
\newzctheorem{example}[theorem]{Example}
%\newzctheorem*{conv} {Convention} 
%\newzctheorem*{nota} {Notation} 
%\newzctheorem*{notas} {Notations} 
\newtheorem*{note}{Note}
%\newzctheorem*{expl} {Explication}
\newzctheorem{question} {Question}

%%%% Proof environnement
%% When trouble with the qed symbol one solution is to put
%% \belowdisplayskip=-12pt  the last align or split environnement.
\renewcommand{\qedsymbol}{$\dashv$}


\zcRefTypeSetup{maintheorem}{
  Name-sg = Main Theorem ,
  name-sg = main theorem ,
  Name-pl = Main Theorems ,
  name-pl = main theorems ,
}

\zcRefTypeSetup{fact}{
  Name-sg = Fact ,
  name-sg = fact ,
  Name-pl = Facts ,
  name-pl = facts ,
}

%%% enumitem definitions

% remove name "item" when referencing items
\zcRefTypeSetup{item}{
    refbounds = {(,,,)} , % add brackets around the linked number label
    Name-sg=,
    name-sg=,
    Name-pl=,
    name-pl=,
    Name-sg-ab=,
    name-sg-ab=,
    Name-pl-ab=,
    name-pl-ab=
}

\zcRefTypeSetup{item}{
}

%\zcsetup{
%        countertype = {
%          enumThmi   = item,
%          enumThmii  = item,
%          enumThm*i   = item ,
%          enumThm*ii  = item ,
%          enumDefni   = item ,
%          enumDefnii  = item ,
%          enumProofi   = item ,
%          enumProofParameteri   = item ,
%          descThm = item,
%          descProof = item,
%          enumStari = item,
%          enumRemsi   = item , 
%},
%counterresetby = {
%          enumDefnii  = enumDefni ,
%	 enumThm*ii  = enumThm*i ,
%          enumThmii  = enumThmi ,
%},
%}



%
%
%
%\newlist{enumThm}{enumerate}{2}% enumerate in Theorems
%\setlist[enumThm,1]{label=\upshape(\roman*)}%beginpenalty=4,
%\setlist[enumThm,2]{label=\upshape(\alph*)}
%
%\newlist{enumThm*}{enumerate*}{2}% inline enumerate in Theorems
%\setlist[enumThm*,1]{label=\upshape(\roman*)}%beginpenalty=4,
%%\setlist[enumThm,2]{label=\upshape(\alph*)}
%
%\newlist{itemThm}{itemize}{1}% itemize in theorems
%\setlist[itemThm]{label=--}
%
%\newlist{enumDefn}{enumerate}{2}% enumerate in Definitions
%\setlist[enumDefn,1]{label=(\arabic*)}
%\setlist[enumDefn,2]{label=(\arabic{enumDefni}\alph*),leftmargin=3em}
%
%\newlist{enumRems}{enumerate}{1}% enumerate in Definitions
%\setlist[enumRems,1]{label=\upshape(\arabic*)}
%
%
%\newlist{itemProof}{itemize}{1}% itemize in Proofs
%\setlist[itemProof]{label=--}
%
%\newlist{enumProof}{enumerate}{1}% enumerate in Proofs
%\setlist[enumProof,1]{label=\upshape(\alph*)}
%
%\newlist{enumProofParameter}{enumerate}{1}% itemize in Proofs
%\setlist[enumProofParameter,1]{label=\upshape(\alph*)$_{\xi}$}
%
%
\newlist{descThm}{description}{1}% Desc in Thm statement
\setlist[descThm]{font=\normalfont}
%
%\newlist{descProof}{description}{1}% Desc in proof statement
%\setlist[descProof]{font={\normalfont\itshape}}
%
%\makeatletter
%\newcommand*{\enumSTAR}[1]{%
%  \expandafter\@enumSTAR\csname c@#1\endcsname%
%}
%
%\newcommand*{\@enumSTAR}[1]{%
%  $\ifcase#1\or \star\or\star\star\or\star\star\star%
%    \else\@ctrerr\fi$%
%}
%\AddEnumerateCounter{\enumSTAR}{\@enumSTAR}{\star}
%\makeatother
%
%\newlist{enumStar}{enumerate}{1}
%\setlist[enumStar]{label=(\enumSTAR*), ref=(\enumSTAR*)}



